Linearization of Monge-Amp\`ere Equations and Statistical Applications

Optimal transport has found numerous applications across data science, many of which require differentiating the optimal transport map with respect to the underlying probability densities in the Fr\'echet sense. In this work, we show that when the reference measure $Q$ is sufficiently regular in space and the curve of target measures $\{P_t\}_{t\in I}$ is both spatially regular and $\mathcal{C}^1$ in time, then the associated curve of optimal transport maps $\{\nabla \phi_t\}_{t\in I}$ pushing $Q$ toward $P_t$ is itself a $\mathcal{C}^1$ curve. Moreover, we identify its time derivative as the solution to the \emph{linearized Monge--Amp\`ere equation}, a second-order elliptic PDE with strictly oblique boundary conditions and a vanishing zero-order term. Our proof relies on applying the implicit function theorem to the Monge--Amp\`ere equation with natural boundary conditions. As consequences, we establish regularity of the transport-based quantile regressor with respect to the covariates and derive a central limit theorem for smooth optimal transport maps.

==> mathsymbols.tex <==
\usepackage{amsfonts,bbm,bm}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\RequirePackage[capitalize]{cleveref}

% Non-italic Latin lower case
\newcommand{\Ta}{\mathrm{a}}
\newcommand{\Tb}{\mathrm{b}}
\newcommand{\Tc}{\mathrm{c}}
\newcommand{\Td}{\mathrm{d}}
\newcommand{\Te}{\mathrm{e}}
\newcommand{\Tf}{\mathrm{f}}
\newcommand{\Tg}{\mathrm{g}}
\newcommand{\Th}{\mathrm{h}}
\newcommand{\Ti}{\mathrm{i}}
\newcommand{\Tj}{\mathrm{j}}
\newcommand{\Tk}{\mathrm{k}}
\newcommand{\Tl}{\mathrm{l}}
\newcommand{\Tm}{\mathrm{m}}
\newcommand{\Tn}{\mathrm{n}}
\newcommand{\To}{\mathrm{o}}
\newcommand{\Tp}{\mathrm{p}}
\newcommand{\Tq}{\mathrm{q}}
\newcommand{\Tr}{\mathrm{r}}
\newcommand{\Ts}{\mathrm{s}}
\newcommand{\Tt}{\mathrm{t}}
\newcommand{\Tu}{\mathrm{u}}
\newcommand{\Tv}{\mathrm{v}}
\newcommand{\Tw}{\mathrm{w}}
\newcommand{\Tx}{\mathrm{x}}
\newcommand{\Ty}{\mathrm{y}}
\newcommand{\Tz}{\mathrm{z}}

% Non-italic Latin upper case
\newcommand{\TA}{\mathrm{A}}
\newcommand{\TB}{\mathrm{B}}
\newcommand{\TC}{\mathrm{C}}
\newcommand{\TD}{\mathrm{D}}
\newcommand{\TE}{\mathrm{E}}
\newcommand{\TF}{\mathrm{F}}
\newcommand{\TG}{\mathrm{G}}
\renewcommand{\TH}{\mathrm{H}}
\newcommand{\TI}{\mathrm{I}}
\newcommand{\TJ}{\mathrm{J}}
\newcommand{\TK}{\mathrm{K}}
\newcommand{\TL}{\mathrm{L}}
\newcommand{\TM}{\mathrm{M}}
\newcommand{\TN}{\mathrm{N}}
\newcommand{\TO}{\mathrm{O}}
\newcommand{\TP}{\mathrm{P}}
\newcommand{\TQ}{\mathrm{Q}}
\newcommand{\TR}{\mathrm{R}}
\newcommand{\TS}{\mathrm{S}}
\newcommand{\TT}{\mathrm{T}}
\newcommand{\TU}{\mathrm{U}}
\newcommand{\TV}{\mathrm{V}}
\newcommand{\TW}{\mathrm{W}}
\newcommand{\TX}{\mathrm{X}}
\newcommand{\TY}{\mathrm{Y}}
\newcommand{\TZ}{\mathrm{Z}}

% 	Bold, non-italic Latin lower case
\newcommand{\Ba}{\mathbf{a}}
\newcommand{\Bb}{\mathbf{b}}
\newcommand{\Bc}{\mathbf{c}}
\newcommand{\Bd}{\mathbf{d}}
\newcommand{\Be}{\mathbf{e}}
\newcommand{\Bf}{\mathbf{f}}
\newcommand{\Bg}{\mathbf{g}}
\newcommand{\Bh}{\mathbf{h}}
\newcommand{\Bi}{\mathbf{i}}
\newcommand{\Bj}{\mathbf{j}}
\newcommand{\Bk}{\mathbf{k}}
\newcommand{\Bl}{\mathbf{l}}
\newcommand{\Bm}{\mathbf{m}}
\newcommand{\Bn}{\mathbf{n}}
\newcommand{\Bo}{\mathbf{o}}
\newcommand{\Bp}{\mathbf{p}}
\newcommand{\Bq}{\mathbf{q}}
\newcommand{\Br}{\mathbf{r}}
\newcommand{\Bs}{\mathbf{s}}
\newcommand{\Bt}{\mathbf{t}}
\newcommand{\Bu}{\mathbf{u}}
\newcommand{\Bv}{\mathbf{v}}
\newcommand{\Bw}{\mathbf{w}}
% \newcommand{\Bx}{\mathbf{x}}
\newcommand{\Bx}{\bm{x}}
\newcommand{\By}{\mathbf{y}}
\newcommand{\Bz}{\mathbf{z}}


%   Some random stuff
\def\d{\, {\rm d}}

% 	Bold, non-italic Latin upper case
\newcommand{\BA}{\mathbf{A}}
\newcommand{\BB}{\mathbf{B}}
\newcommand{\BC}{\mathbf{C}}
\newcommand{\BD}{\mathbf{D}}
\newcommand{\BE}{\mathbf{E}}
\newcommand{\BF}{\mathbf{F}}
\newcommand{\BG}{\mathbf{G}}
\newcommand{\BH}{\mathbf{H}}
\newcommand{\BI}{\mathbf{I}}
\newcommand{\BJ}{\mathbf{J}}
\newcommand{\BK}{\mathbf{K}}
\newcommand{\BL}{\mathbf{L}}
\newcommand{\BM}{\mathbf{M}}
\newcommand{\BN}{\mathbf{N}}
\newcommand{\BO}{\mathbf{O}}
\newcommand{\BP}{\mathbf{P}}
\newcommand{\BQ}{\mathbf{Q}}
\newcommand{\BR}{\mathbf{R}}
\newcommand{\BS}{\mathbf{S}}
\newcommand{\BT}{\mathbf{T}}
\newcommand{\BU}{\mathbf{U}}
\newcommand{\BV}{\mathbf{V}}
\newcommand{\BW}{\mathbf{W}}
\newcommand{\BX}{\mathbf{X}}
\newcommand{\BY}{\mathbf{Y}}
\newcommand{\BZ}{\mathbf{Z}}

%	Bold, italic Latin lower case
\newcommand{\BIa}{{\boldsymbol{a}}}
\newcommand{\BIb}{{\boldsymbol{b}}}
\newcommand{\BIc}{{\boldsymbol{c}}}
\newcommand{\BId}{{\boldsymbol{d}}}
\newcommand{\BIe}{{\boldsymbol{e}}}
\newcommand{\BIf}{{\boldsymbol{f}}}
\newcommand{\BIg}{{\boldsymbol{g}}}
\newcommand{\BIh}{{\boldsymbol{h}}}
\newcommand{\BIi}{{\boldsymbol{i}}}
\newcommand{\BIj}{{\boldsymbol{j}}}
\newcommand{\BIk}{{\boldsymbol{k}}}
\newcommand{\BIl}{{\boldsymbol{l}}}
\newcommand{\BIm}{{\boldsymbol{m}}}
\newcommand{\BIn}{{\boldsymbol{n}}}
\newcommand{\BIo}{{\boldsymbol{o}}}
\newcommand{\BIp}{{\boldsymbol{p}}}
\newcommand{\BIq}{{\boldsymbol{q}}}
\newcommand{\BIr}{{\boldsymbol{r}}}
\newcommand{\BIs}{{\boldsymbol{s}}}
\newcommand{\BIt}{{\boldsymbol{t}}}
\newcommand{\BIu}{{\boldsymbol{u}}}
\newcommand{\BIv}{{\boldsymbol{v}}}
\newcommand{\BIw}{{\boldsymbol{w}}}
\newcommand{\BIx}{{\boldsymbol{x}}}
\newcommand{\BIy}{{\boldsymbol{y}}}
\newcommand{\BIz}{{\boldsymbol{z}}}

%	Bold, italic Latin upper case
\newcommand{\BIA}{{\boldsymbol{A}}}
\newcommand{\BIB}{{\boldsymbol{B}}}
\newcommand{\BIC}{{\boldsymbol{C}}}
\newcommand{\BID}{{\boldsymbol{D}}}
\newcommand{\BIE}{{\boldsymbol{E}}}
\newcommand{\BIF}{{\boldsymbol{F}}}
\newcommand{\BIG}{{\boldsymbol{G}}}
\newcommand{\BIH}{{\boldsymbol{H}}}
\newcommand{\BII}{{\boldsymbol{I}}}
\newcommand{\BIJ}{{\boldsymbol{J}}}
\newcommand{\BIK}{{\boldsymbol{K}}}
\newcommand{\BIL}{{\boldsymbol{L}}}
\newcommand{\BIM}{{\boldsymbol{M}}}
\newcommand{\BIN}{{\boldsymbol{N}}}
\newcommand{\BIO}{{\boldsymbol{O}}}
\newcommand{\BIP}{{\boldsymbol{P}}}
\newcommand{\BIQ}{{\boldsymbol{Q}}}
\newcommand{\BIR}{{\boldsymbol{R}}}
\newcommand{\BIS}{{\boldsymbol{S}}}
\newcommand{\BIT}{{\boldsymbol{T}}}
\newcommand{\BIU}{{\boldsymbol{U}}}
\newcommand{\BIV}{{\boldsymbol{V}}}
\newcommand{\BIW}{{\boldsymbol{W}}}
\newcommand{\BIX}{{\boldsymbol{X}}}
\newcommand{\BIY}{{\boldsymbol{Y}}}
\newcommand{\BIZ}{{\boldsymbol{Z}}}

%	Caligraphic, italic Latin upper case
\newcommand{\CA}{\mathcal{A}}
\newcommand{\CB}{\mathcal{B}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\CD}{\mathcal{D}}
\newcommand{\CE}{\mathcal{E}}
\newcommand{\CF}{\mathcal{F}}
\newcommand{\CG}{\mathcal{G}}
\newcommand{\CH}{\mathcal{H}}
\newcommand{\CI}{\mathcal{I}}
\newcommand{\CJ}{\mathcal{J}}
\newcommand{\CK}{\mathcal{K}}
\newcommand{\CL}{\mathcal{L}}
\newcommand{\CM}{\mathcal{M}}
\newcommand{\CN}{\mathcal{N}}
\newcommand{\CO}{\mathcal{O}}
\newcommand{\CP}{\mathcal{P}}
\newcommand{\CQ}{\mathcal{Q}}
\newcommand{\CR}{\mathcal{R}}
\newcommand{\CS}{\mathcal{S}}
\newcommand{\CT}{\mathcal{T}}
\newcommand{\CU}{\mathcal{U}}
\newcommand{\CV}{\mathcal{V}}
\newcommand{\CW}{\mathcal{W}}
\newcommand{\CX}{\mathcal{X}}
\newcommand{\CY}{\mathcal{Y}}
\newcommand{\CZ}{\mathcal{Z}}

\newcommand{\CXt}{\mathcal{X}_t}
\newcommand{\CYt}{\mathcal{Y}_t}

%	Bold, caligraphic, italic Latin upper case
\newcommand{\BCA}{{\boldsymbol{\mathcal{A}}}}
\newcommand{\BCB}{{\boldsymbol{\mathcal{B}}}}
\newcommand{\BCC}{{\boldsymbol{\mathcal{C}}}}
\newcommand{\BCD}{{\boldsymbol{\mathcal{D}}}}
\newcommand{\BCE}{{\boldsymbol{\mathcal{E}}}}
\newcommand{\BCF}{{\boldsymbol{\mathcal{F}}}}
\newcommand{\BCG}{{\boldsymbol{\mathcal{G}}}}
\newcommand{\BCH}{{\boldsymbol{\mathcal{H}}}}
\newcommand{\BCI}{{\boldsymbol{\mathcal{I}}}}
\newcommand{\BCJ}{{\boldsymbol{\mathcal{J}}}}
\newcommand{\BCK}{{\boldsymbol{\mathcal{K}}}}
\newcommand{\BCL}{{\boldsymbol{\mathcal{L}}}}
\newcommand{\BCM}{{\boldsymbol{\mathcal{M}}}}
\newcommand{\BCN}{{\boldsymbol{\mathcal{N}}}}
\newcommand{\BCO}{{\boldsymbol{\mathcal{O}}}}
\newcommand{\BCP}{{\boldsymbol{\mathcal{P}}}}
\newcommand{\BCQ}{{\boldsymbol{\mathcal{Q}}}}
\newcommand{\BCR}{{\boldsymbol{\mathcal{R}}}}
\newcommand{\BCS}{{\boldsymbol{\mathcal{S}}}}
\newcommand{\BCT}{{\boldsymbol{\mathcal{T}}}}
\newcommand{\BCU}{{\boldsymbol{\mathcal{U}}}}
\newcommand{\BCV}{{\boldsymbol{\mathcal{V}}}}
\newcommand{\BCW}{{\boldsymbol{\mathcal{W}}}}
\newcommand{\BCX}{{\boldsymbol{\mathcal{X}}}}
\newcommand{\BCY}{{\boldsymbol{\mathcal{Y}}}}
\newcommand{\BCZ}{{\boldsymbol{\mathcal{Z}}}}

%	Fractur, non-italic Latin upper case
\newcommand{\FA}{\mathfrak{A}}
\newcommand{\FB}{\mathfrak{B}}
\newcommand{\FC}{\mathfrak{C}}
\newcommand{\FD}{\mathfrak{D}}
\newcommand{\FE}{\mathfrak{E}}
\newcommand{\FF}{\mathfrak{F}}
\newcommand{\FG}{\mathfrak{G}}
\newcommand{\FH}{\mathfrak{H}}
\newcommand{\FI}{\mathfrak{I}}
\newcommand{\FJ}{\mathfrak{J}}
\newcommand{\FK}{\mathfrak{K}}
\newcommand{\FL}{\mathfrak{L}}
\newcommand{\FM}{\mathfrak{M}}
\newcommand{\FN}{\mathfrak{N}}
\newcommand{\FO}{\mathfrak{O}}
\newcommand{\FP}{\mathfrak{P}}
\newcommand{\FQ}{\mathfrak{Q}}
\newcommand{\FR}{\mathfrak{R}}
\newcommand{\FS}{\mathfrak{S}}
\newcommand{\FT}{\mathfrak{T}}
\newcommand{\FU}{\mathfrak{U}}
\newcommand{\FV}{\mathfrak{V}}
\newcommand{\FW}{\mathfrak{W}}
\newcommand{\FX}{\mathfrak{X}}
\newcommand{\FY}{\mathfrak{Y}}
\newcommand{\FZ}{\mathfrak{Z}}

%	Fractur, non-italic Latin lower case
\newcommand{\Fa}{\mathfrak{a}}
\newcommand{\Fb}{\mathfrak{b}}
\newcommand{\Fc}{\mathfrak{c}}
\newcommand{\Fd}{\mathfrak{d}}
\newcommand{\Fe}{\mathfrak{e}}
\newcommand{\Ff}{\mathfrak{f}}
\newcommand{\Fg}{\mathfrak{g}}
\newcommand{\Fh}{\mathfrak{h}}
\newcommand{\Fi}{\mathfrak{i}}
\newcommand{\Fj}{\mathfrak{j}}
\newcommand{\Fk}{\mathfrak{k}}
\newcommand{\Fl}{\mathfrak{l}}
\newcommand{\Fm}{\mathfrak{m}}
\newcommand{\Fn}{\mathfrak{n}}
\newcommand{\Fo}{\mathfrak{o}}
\newcommand{\Fp}{\mathfrak{p}}
\newcommand{\Fq}{\mathfrak{q}}
\newcommand{\Fr}{\mathfrak{r}}
\newcommand{\Fs}{\mathfrak{s}}
\newcommand{\Ft}{\mathfrak{t}}
\newcommand{\Fu}{\mathfrak{u}}
\newcommand{\Fv}{\mathfrak{v}}
\newcommand{\Fw}{\mathfrak{w}}
\newcommand{\Fx}{\mathfrak{x}}
\newcommand{\Fy}{\mathfrak{y}}
\newcommand{\Fz}{\mathfrak{z}}

%	Bold, Fractur, non-italic Latin upper case
\newcommand{\BFA}{\boldsymbol{\mathfrak{A}}}
\newcommand{\BFB}{\boldsymbol{\mathfrak{B}}}
\newcommand{\BFC}{\boldsymbol{\mathfrak{C}}}
\newcommand{\BFD}{\boldsymbol{\mathfrak{D}}}
\newcommand{\BFE}{\boldsymbol{\mathfrak{E}}}
\newcommand{\BFF}{\boldsymbol{\mathfrak{F}}}
\newcommand{\BFG}{\boldsymbol{\mathfrak{G}}}
\newcommand{\BFH}{\boldsymbol{\mathfrak{H}}}
\newcommand{\BFI}{\boldsymbol{\mathfrak{I}}}
\newcommand{\BFJ}{\boldsymbol{\mathfrak{J}}}
\newcommand{\BFK}{\boldsymbol{\mathfrak{K}}}
\newcommand{\BFL}{\boldsymbol{\mathfrak{L}}}
\newcommand{\BFM}{\boldsymbol{\mathfrak{M}}}
\newcommand{\BFN}{\boldsymbol{\mathfrak{N}}}
\newcommand{\BFO}{\boldsymbol{\mathfrak{O}}}
\newcommand{\BFP}{\boldsymbol{\mathfrak{P}}}
\newcommand{\BFQ}{\boldsymbol{\mathfrak{Q}}}
\newcommand{\BFR}{\boldsymbol{\mathfrak{R}}}
\newcommand{\BFS}{\boldsymbol{\mathfrak{S}}}
\newcommand{\BFT}{\boldsymbol{\mathfrak{T}}}
\newcommand{\BFU}{\boldsymbol{\mathfrak{U}}}
\newcommand{\BFV}{\boldsymbol{\mathfrak{V}}}
\newcommand{\BFW}{\boldsymbol{\mathfrak{W}}}
\newcommand{\BFX}{\boldsymbol{\mathfrak{X}}}
\newcommand{\BFY}{\boldsymbol{\mathfrak{Y}}}
\newcommand{\BFZ}{\boldsymbol{\mathfrak{Z}}}

%	Bold, Fractur, non-italic Latin lower case
\newcommand{\BFa}{\boldsymbol{\mathfrak{a}}}
\newcommand{\BFb}{\boldsymbol{\mathfrak{b}}}
\newcommand{\BFc}{\boldsymbol{\mathfrak{c}}}
\newcommand{\BFd}{\boldsymbol{\mathfrak{d}}}
\newcommand{\BFe}{\boldsymbol{\mathfrak{e}}}
\newcommand{\BFf}{\boldsymbol{\mathfrak{f}}}
\newcommand{\BFg}{\boldsymbol{\mathfrak{g}}}
\newcommand{\BFh}{\boldsymbol{\mathfrak{h}}}
\newcommand{\BFi}{\boldsymbol{\mathfrak{i}}}
\newcommand{\BFj}{\boldsymbol{\mathfrak{j}}}
\newcommand{\BFk}{\boldsymbol{\mathfrak{k}}}
\newcommand{\BFl}{\boldsymbol{\mathfrak{l}}}
\newcommand{\BFm}{\boldsymbol{\mathfrak{m}}}
\newcommand{\BFn}{\boldsymbol{\mathfrak{n}}}
\newcommand{\BFo}{\boldsymbol{\mathfrak{o}}}
\newcommand{\BFp}{\boldsymbol{\mathfrak{p}}}
\newcommand{\BFq}{\boldsymbol{\mathfrak{q}}}
\newcommand{\BFr}{\boldsymbol{\mathfrak{r}}}
\newcommand{\BFs}{\boldsymbol{\mathfrak{s}}}
\newcommand{\BFt}{\boldsymbol{\mathfrak{t}}}
\newcommand{\BFu}{\boldsymbol{\mathfrak{u}}}
\newcommand{\BFv}{\boldsymbol{\mathfrak{v}}}
\newcommand{\BFw}{\boldsymbol{\mathfrak{w}}}
\newcommand{\BFx}{\boldsymbol{\mathfrak{x}}}
\newcommand{\BFy}{\boldsymbol{\mathfrak{y}}}
\newcommand{\BFz}{\boldsymbol{\mathfrak{z}}}

%	Boondox caligraphic, italic Latin upper case
\newcommand{\DCA}{\mathscr{A}}
\newcommand{\DCB}{\mathscr{B}}
\newcommand{\DCC}{\mathscr{C}}
\newcommand{\DCD}{\mathscr{D}}
\newcommand{\DCE}{\mathscr{E}}
\newcommand{\DCF}{\mathscr{F}}
\newcommand{\DCG}{\mathscr{G}}
\newcommand{\DCH}{\mathscr{H}}
\newcommand{\DCI}{\mathscr{I}}
\newcommand{\DCJ}{\mathscr{J}}
\newcommand{\DCK}{\mathscr{K}}
\newcommand{\DCL}{\mathscr{L}}
\newcommand{\DCM}{\mathscr{M}}
\newcommand{\DCN}{\mathscr{N}}
\newcommand{\DCO}{\mathscr{O}}
\newcommand{\DCP}{\mathscr{P}}
\newcommand{\DCQ}{\mathscr{Q}}
\newcommand{\DCR}{\mathscr{R}}
\newcommand{\DCS}{\mathscr{S}}
\newcommand{\DCT}{\mathscr{T}}
\newcommand{\DCU}{\mathscr{U}}
\newcommand{\DCV}{\mathscr{V}}
\newcommand{\DCW}{\mathscr{W}}
\newcommand{\DCX}{\mathscr{X}}
\newcommand{\DCY}{\mathscr{Y}}
\newcommand{\DCZ}{\mathscr{Z}}

%	Bold, Boondox caligraphic, italic Latin upper case
\newcommand{\BDCA}{{\boldsymbol{\mathscr{A}}}}
\newcommand{\BDCB}{{\boldsymbol{\mathscr{B}}}}
\newcommand{\BDCC}{{\boldsymbol{\mathscr{C}}}}
\newcommand{\BDCD}{{\boldsymbol{\mathscr{D}}}}
\newcommand{\BDCE}{{\boldsymbol{\mathscr{E}}}}
\newcommand{\BDCF}{{\boldsymbol{\mathscr{F}}}}
\newcommand{\BDCG}{{\boldsymbol{\mathscr{G}}}}
\newcommand{\BDCH}{{\boldsymbol{\mathscr{H}}}}
\newcommand{\BDCI}{{\boldsymbol{\mathscr{I}}}}
\newcommand{\BDCJ}{{\boldsymbol{\mathscr{J}}}}
\newcommand{\BDCK}{{\boldsymbol{\mathscr{K}}}}
\newcommand{\BDCL}{{\boldsymbol{\mathscr{L}}}}
\newcommand{\BDCM}{{\boldsymbol{\mathscr{M}}}}
\newcommand{\BDCN}{{\boldsymbol{\mathscr{N}}}}
\newcommand{\BDCO}{{\boldsymbol{\mathscr{O}}}}
\newcommand{\BDCP}{{\boldsymbol{\mathscr{P}}}}
\newcommand{\BDCQ}{{\boldsymbol{\mathscr{Q}}}}
\newcommand{\BDCR}{{\boldsymbol{\mathscr{R}}}}
\newcommand{\BDCS}{{\boldsymbol{\mathscr{S}}}}
\newcommand{\BDCT}{{\boldsymbol{\mathscr{T}}}}
\newcommand{\BDCU}{{\boldsymbol{\mathscr{U}}}}
\newcommand{\BDCV}{{\boldsymbol{\mathscr{V}}}}
\newcommand{\BDCW}{{\boldsymbol{\mathscr{W}}}}
\newcommand{\BDCX}{{\boldsymbol{\mathscr{X}}}}
\newcommand{\BDCY}{{\boldsymbol{\mathscr{Y}}}}
\newcommand{\BDCZ}{{\boldsymbol{\mathscr{Z}}}}

%	San-serif upper base
\newcommand{\SFA}{\mathsf{A}}
\newcommand{\SFB}{\mathsf{B}}
\newcommand{\SFC}{\mathsf{C}}
\newcommand{\SFD}{\mathsf{D}}
\newcommand{\SFE}{\mathsf{E}}
\newcommand{\SFF}{\mathsf{F}}
\newcommand{\SFG}{\mathsf{G}}
\newcommand{\SFH}{\mathsf{H}}
\newcommand{\SFI}{\mathsf{I}}
\newcommand{\SFJ}{\mathsf{J}}
\newcommand{\SFK}{\mathsf{K}}
\newcommand{\SFL}{\mathsf{L}}
\newcommand{\SFM}{\mathsf{M}}
\newcommand{\SFN}{\mathsf{N}}
\newcommand{\SFO}{\mathsf{O}}
\newcommand{\SFP}{\mathsf{P}}
\newcommand{\SFQ}{\mathsf{Q}}
\newcommand{\SFR}{\mathsf{R}}
\newcommand{\SFS}{\mathsf{S}}
\newcommand{\SFT}{\mathsf{T}}
\newcommand{\SFU}{\mathsf{U}}
\newcommand{\SFV}{\mathsf{V}}
\newcommand{\SFW}{\mathsf{W}}
\newcommand{\SFX}{\mathsf{X}}
\newcommand{\SFY}{\mathsf{Y}}
\newcommand{\SFZ}{\mathsf{Z}}

%	San-serif lower base
\newcommand{\SFa}{\mathsf{a}}
\newcommand{\SFb}{\mathsf{b}}
\newcommand{\SFc}{\mathsf{c}}
\newcommand{\SFd}{\mathsf{d}}
\newcommand{\SFe}{\mathsf{e}}
\newcommand{\SFf}{\mathsf{f}}
\newcommand{\SFg}{\mathsf{g}}
\newcommand{\SFh}{\mathsf{h}}
\newcommand{\SFi}{\mathsf{i}}
\newcommand{\SFj}{\mathsf{j}}
\newcommand{\SFk}{\mathsf{k}}
\newcommand{\SFl}{\mathsf{l}}
\newcommand{\SFm}{\mathsf{m}}
\newcommand{\SFn}{\mathsf{n}}
\newcommand{\SFo}{\mathsf{o}}
\newcommand{\SFp}{\mathsf{p}}
\newcommand{\SFq}{\mathsf{q}}
\newcommand{\SFr}{\mathsf{r}}
\newcommand{\SFs}{\mathsf{s}}
\newcommand{\SFt}{\mathsf{t}}
\newcommand{\SFu}{\mathsf{u}}
\newcommand{\SFv}{\mathsf{v}}
\newcommand{\SFw}{\mathsf{w}}
\newcommand{\SFx}{\mathsf{x}}
\newcommand{\SFy}{\mathsf{y}}
\newcommand{\SFz}{\mathsf{z}}

%	Monospace upper base
\newcommand{\TTA}{\mathtt{A}}
\newcommand{\TTB}{\mathtt{B}}
\newcommand{\TTC}{\mathtt{C}}
\newcommand{\TTD}{\mathtt{D}}
\newcommand{\TTE}{\mathtt{E}}
\newcommand{\TTF}{\mathtt{F}}
\newcommand{\TTG}{\mathtt{G}}
\newcommand{\TTH}{\mathtt{H}}
\newcommand{\TTI}{\mathtt{I}}
\newcommand{\TTJ}{\mathtt{J}}
\newcommand{\TTK}{\mathtt{K}}
\newcommand{\TTL}{\mathtt{L}}
\newcommand{\TTM}{\mathtt{M}}
\newcommand{\TTN}{\mathtt{N}}
\newcommand{\TTO}{\mathtt{O}}
\newcommand{\TTP}{\mathtt{P}}
\newcommand{\TTQ}{\mathtt{Q}}
\newcommand{\TTR}{\mathtt{R}}
\newcommand{\TTS}{\mathtt{S}}
\newcommand{\TTT}{\mathtt{T}}
\newcommand{\TTU}{\mathtt{U}}
\newcommand{\TTV}{\mathtt{V}}
\newcommand{\TTW}{\mathtt{W}}
\newcommand{\TTX}{\mathtt{X}}
\newcommand{\TTY}{\mathtt{Y}}
\newcommand{\TTZ}{\mathtt{Z}}

%	San-serif lower base
\newcommand{\TTa}{\mathtt{a}}
\newcommand{\TTb}{\mathtt{b}}
\newcommand{\TTc}{\mathtt{c}}
\newcommand{\TTd}{\mathtt{d}}
\newcommand{\TTe}{\mathtt{e}}
\newcommand{\TTf}{\mathtt{f}}
\newcommand{\TTg}{\mathtt{g}}
\newcommand{\TTh}{\mathtt{h}}
\newcommand{\TTi}{\mathtt{i}}
\newcommand{\TTj}{\mathtt{j}}
\newcommand{\TTk}{\mathtt{k}}
\newcommand{\TTl}{\mathtt{l}}
\newcommand{\TTm}{\mathtt{m}}
\newcommand{\TTn}{\mathtt{n}}
\newcommand{\TTo}{\mathtt{o}}
\newcommand{\TTp}{\mathtt{p}}
\newcommand{\TTq}{\mathtt{q}}
\newcommand{\TTr}{\mathtt{r}}
\newcommand{\TTs}{\mathtt{s}}
\newcommand{\TTt}{\mathtt{t}}
\newcommand{\TTu}{\mathtt{u}}
\newcommand{\TTv}{\mathtt{v}}
\newcommand{\TTw}{\mathtt{w}}
\newcommand{\TTx}{\mathtt{x}}
\newcommand{\TTy}{\mathtt{y}}
\newcommand{\TTz}{\mathtt{z}}

% Non-italic Greek upper case
\newcommand{\Alpha}{\mathrm{A}}
\newcommand{\TBeta}{\mathrm{B}} % Conflict with \Beta
\newcommand{\Epsilon}{\mathrm{E}}
\newcommand{\Zeta}{\mathrm{Z}}
\newcommand{\Eta}{\mathrm{H}}
\newcommand{\Iota}{\mathrm{I}}
\newcommand{\Kappa}{\mathrm{K}}
\newcommand{\Mu}{\mathrm{M}}
\newcommand{\Nu}{\mathrm{N}}
\newcommand{\Omikron}{\mathrm{O}}
\newcommand{\Rho}{\mathrm{P}}
\newcommand{\Tau}{\mathrm{T}}
\newcommand{\Chi}{\mathrm{X}}

% Italic Greek upper case
\newcommand{\IAlpha}{A}
\newcommand{\IBeta}{B}
\newcommand{\IGamma}{\mathit{\Gamma}}
\newcommand{\IDelta}{\mathit{\Delta}}
\newcommand{\IEpsilon}{E}
\newcommand{\IZeta}{Z}
\newcommand{\IEta}{H}
\newcommand{\ITheta}{\mathit{\Theta}}
\newcommand{\IIota}{I}
\newcommand{\IKappa}{K}
\newcommand{\ILambda}{\mathit{\Lambda}}
\newcommand{\IMu}{M}
\newcommand{\INu}{N}
\newcommand{\IXi}{\mathit{\Xi}}
\newcommand{\IOmikron}{O}
\newcommand{\IPi}{\mathit{\Pi}}
\newcommand{\IRho}{P}
\newcommand{\ISigma}{\mathit{\Sigma}}
\newcommand{\ITau}{T}
\newcommand{\IUpsilon}{\mathit{\Upsilon}}
\newcommand{\IPhi}{\mathit{\Phi}}
\newcommand{\IChi}{X}
\newcommand{\IPsi}{\mathit{\Psi}}
\newcommand{\IOmega}{\mathit{\Omega}}

% Italic Greek lower case
\newcommand{\omikron}{o}

% Bold, non-italic Greek upper case
\newcommand{\BAlpha}{{\boldsymbol{\Alpha}}}
\newcommand{\BBeta}{{\boldsymbol{\Beta}}}
\newcommand{\BGamma}{{\boldsymbol{\Gamma}}}
\newcommand{\BDelta}{{\boldsymbol{\Delta}}}
\newcommand{\BEpsilon}{{\boldsymbol{\Epsilon}}}
\newcommand{\BZeta}{{\boldsymbol{\Zeta}}}
\newcommand{\BEta}{{\boldsymbol{\Eta}}}
\newcommand{\BTheta}{{\boldsymbol{\Theta}}}
\newcommand{\BIota}{{\boldsymbol{\Iota}}}
\newcommand{\BKappa}{{\boldsymbol{\Kappa}}}
\newcommand{\BLambda}{{\boldsymbol{\Lambda}}}
\newcommand{\BMu}{{\boldsymbol{\Mu}}}
\newcommand{\BNu}{{\boldsymbol{\Nu}}}
\newcommand{\BXi}{{\boldsymbol{\Xi}}}
\newcommand{\BOmikron}{{\boldsymbol{\Omikron}}}
\newcommand{\BPi}{{\boldsymbol{\Pi}}}
\newcommand{\BRho}{{\boldsymbol{\Rho}}}
\newcommand{\BSigma}{{\boldsymbol{\Sigma}}}
\newcommand{\BTau}{{\boldsymbol{\Tau}}}
\newcommand{\BUpsilon}{{\boldsymbol{\Upsilon}}}
\newcommand{\BPhi}{{\boldsymbol{\Phi}}}
\newcommand{\BChi}{{\boldsymbol{\Chi}}}
\newcommand{\BPsi}{{\boldsymbol{\Psi}}}
\newcommand{\BOmega}{{\boldsymbol{\Omega}}}

% Bold, italic Greek upper case
\newcommand{\BIAlpha}{{\boldsymbol{\IAlpha}}}
\newcommand{\BIBeta}{{\boldsymbol{\IBeta}}}
\newcommand{\BIGamma}{{\boldsymbol{\IGamma}}}
\newcommand{\BIDelta}{{\boldsymbol{\IDelta}}}
\newcommand{\BIEpsilon}{{\boldsymbol{\IEpsilon}}}
\newcommand{\BIZeta}{{\boldsymbol{\IZeta}}}
\newcommand{\BIEta}{{\boldsymbol{\IEta}}}
\newcommand{\BITheta}{{\boldsymbol{\ITheta}}}
\newcommand{\BIIota}{{\boldsymbol{\IIota}}}
\newcommand{\BIKappa}{{\boldsymbol{\IKappa}}}
\newcommand{\BILambda}{{\boldsymbol{\ILambda}}}
\newcommand{\BIMu}{{\boldsymbol{\IMu}}}
\newcommand{\BINu}{{\boldsymbol{\INu}}}
\newcommand{\BIXi}{{\boldsymbol{\IXi}}}
\newcommand{\BIOmikron}{{\boldsymbol{\IOmikron}}}
\newcommand{\BIPi}{{\boldsymbol{\IPi}}}
\newcommand{\BIRho}{{\boldsymbol{\IRho}}}
\newcommand{\BISigma}{{\boldsymbol{\ISigma}}}
\newcommand{\BITau}{{\boldsymbol{\ITau}}}
\newcommand{\BIUpsilon}{{\boldsymbol{\IUpsilon}}}
\newcommand{\BIPhi}{{\boldsymbol{\IPhi}}}
\newcommand{\BIChi}{{\boldsymbol{\IChi}}}
\newcommand{\BIPsi}{{\boldsymbol{\IPsi}}}
\newcommand{\BIOmega}{{\boldsymbol{\IOmega}}}

% Bold, italic Greek lower case
\newcommand{\Balpha}{{\boldsymbol{\alpha}}}
\newcommand{\Bbeta}{{\boldsymbol{\beta}}}
\newcommand{\Bgamma}{{\boldsymbol{\gamma}}}
\newcommand{\Bdelta}{{\boldsymbol{\delta}}}
\newcommand{\Bepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\Bzeta}{{\boldsymbol{\zeta}}}
\newcommand{\Beta}{{\boldsymbol{\eta}}}
\newcommand{\Btheta}{{\boldsymbol{\theta}}}
\newcommand{\Biota}{{\boldsymbol{\iota}}}
\newcommand{\Bkappa}{{\boldsymbol{\kappa}}}
\newcommand{\Blambda}{{\boldsymbol{\lambda}}}
\newcommand{\Bmu}{{\boldsymbol{\mu}}}
\newcommand{\Bnu}{{\boldsymbol{\nu}}}
\newcommand{\Bxi}{{\boldsymbol{\xi}}}
\newcommand{\Bomikron}{{\boldsymbol{\omikron}}}
\newcommand{\Bpi}{{\boldsymbol{\pi}}}
\newcommand{\Brho}{{\boldsymbol{\rho}}}
\newcommand{\Bsigma}{{\boldsymbol{\sigma}}}
\newcommand{\Btau}{{\boldsymbol{\tau}}}
\newcommand{\Bupsilon}{{\boldsymbol{\upsilon}}}
\newcommand{\Bphi}{{\boldsymbol{\phi}}}
\newcommand{\Bchi}{{\boldsymbol{\chi}}}
\newcommand{\Bpsi}{{\boldsymbol{\psi}}}
\newcommand{\Bomega}{{\boldsymbol{\omega}}}
\newcommand{\Bvarepsilon}{{\boldsymbol{\varepsilon}}}
\newcommand{\Bvarphi}{{\boldsymbol{\varphi}}}
\newcommand{\Bvarpi}{{\boldsymbol{\varpi}}}
\newcommand{\Bvarrho}{{\boldsymbol{\varrho}}}
\newcommand{\Bvarsigma}{{\boldsymbol{\varsigma}}}
\newcommand{\Bvartheta}{{\boldsymbol{\vartheta}}}

% Commonly used symbols
\newcommand{\NORMAL}{\CN} % Normal distribution
\newcommand{\MVNORMAL}{\CM\CV\CN} % Normal distribution
\newcommand{\GP}{\mathcal{GP}} % Gaussian process
% \newcommand{\R}{\mathbb{R}} % real number
% \newcommand{\Q}{\mathbb{Q}} % rational number
% \newcommand{\Z}{\mathbb{Z}} % integer
% \newcommand{\N}{\mathbb{N}} % natural number
%  \newcommand{\T}{\mathbb{T}} % natural number
% \newcommand{\C}{\mathbb{C}} % complex number
\newcommand{\vecone}{\mathbf{1}} % vector of ones
\newcommand{\veczero}{\mathbf{0}} % vector of zeros
\newcommand{\vecinfty}{\boldsymbol{\infty}} % vector of infinities
\newcommand{\INDI}{\mathbbm{1}} % indicator function
\newcommand{\TRANSP}{\mathsf{T}} % transpose
\newcommand{\DIFF}{\Td} % differentiation sign
\newcommand{\DIFFX}[1]{\,\Td{#1}} % differentiation with a measure or a variable name
\newcommand{\DIFFM}[2]{\,{#1}\!\left({#2}\right)} % differentiation with a measure and a variable
\newcommand{\lspan}{\overline{\mathrm{span}}} % span
% \newcommand{\diag}{\mathrm{diag}} % diagonal
\newcommand{\logistic}{\mathrm{logistic}} % logistic transformation
\newcommand{\logit}{\mathrm{logit}} % logit transformation
\newcommand{\PROB}{\mathbb{P}} % probability measure
\newcommand{\PR}{\mathrm{Pr}} % probability
\newcommand{\EXP}{\mathbb{E}} % expectation
\newcommand{\VAR}{\mathrm{Var}} % variance
\newcommand{\COV}{\mathrm{Cov}} % covariance
\newcommand{\CORR}{\mathrm{Corr}} % correlation
\newcommand{\MOD}{\mathrm{mod}} % modulo
\newcommand{\realpart}{\mathrm{Re}} % real part
\newcommand{\imagpart}{\mathrm{Im}} % imaginary part
\newcommand{\clos}{\mathrm{cl}} % closure
\newcommand{\inter}[1]{\mathrm{int}(#1)} % interior
\newcommand{\relint}{\mathrm{relint}} % relative interior
\newcommand{\relbd}{\mathrm{relbd}} % relative boundary
\newcommand{\support}{\mathrm{supp}} % support (of measure)
\newcommand{\conv}{\mathrm{conv}} % convex hull
\newcommand{\aff}{\mathrm{aff}} % affine hull
\newcommand{\cone}{\mathrm{cone}} % conic hull
\newcommand{\dual}{\mathrm{dual}} % dual cone
\newcommand{\dom}{\mathrm{dom}} % domain
\newcommand{\epigraph}{\mathrm{epi}} % epigraph
\newcommand{\tr}{\mathrm{tr}} % trace
\newcommand{\norm}[1]{\left\lVert #1 \right\rVert}
\newcommand{\diver}[1]{\,\mathrm{div}(#1)}
\newcommand{\diam}[1]{\mathrm{diam}(#1)}
% \newcommand{\Id}{\mathrm{Id}}
\newcommand{\range}{\mathrm{Range}}
\newcommand{\Unif}{\mathrm{Unif}}
\newcommand{\vae}{\varepsilon}
\newcommand{\density}[2]{\frac{d#1}{d#2}}
\newcommand{\logden}[2]{\log\left(frac{d#1}{d#2}\right)}
% Roman numbers
\newcommand{\rom}[1]{%
  \textup{\uppercase\expandafter{\romannumeral#1}}%
}
\newcommand{\law}{\mathrm{Law}}
\newcommand{\inner}[2]{\left\langle #1,#2\right\rangle}
\newcommand{\coker}[1]{\text{coker}(#1)}
\newcommand{\kernel}[1]{\text{ker}(#1)}
\newcommand{\im}[1]{\text{im}(#1)}
\newcommand{\ix}[1]{\text{index}(#1)}
\newcommand{\spt}{\text{spt}}
\newcommand{\Tan}{\mathrm{Tan}}
\newcommand{\QV}[1]{\langle #1\rangle}
\newcommand{\qqquad}{\quad\quad\quad}
% \newcommand{\span}[1]{\overline{\mathrm{span}}\{#1\}}

% text color
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\purple}[1]{\textcolor{purple}{#1}}


% Math operators
\DeclareMathOperator*{\argmin}{arg\,min} % argument that minimizes
\DeclareMathOperator*{\argmax}{arg\,max} % argument that maximizes
\DeclareMathOperator*{\minimize}{\mathrm{minimize}} % minimize, for optimization problems
\DeclareMathOperator*{\maximize}{\mathrm{maximize}} % maximize, for optimization problems


% Theorems
% \newtheorem{theorem}{\noindent \textbf{Theorem}}
% \newtheorem{lemma}[theorem]{\noindent \textbf{Lemma}}
% \newtheorem{definition}[theorem]{\noindent \textbf{Definition}}
% \newtheorem{proposition}[theorem]{\noindent \textbf{Proposition}}
% \newtheorem{example}[theorem]{\noindent \textbf{Example}}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{remark}[theorem]{Remark}
% \newtheorem{assumption}[theorem]{Assumption}
% \newtheorem{exmp}[theorem]{Example}
% \numberwithin{theorem}{section}

\newcommand{\Hnull}{\mathcal{H}_0}
\newcommand{\Halt}{\mathcal{H}_1}
\newcommand{\TODO}[1]{\textcolor{red}{#1}}

% PDE related
\newcommand{\ssubset}{\subset\joinrel\subset}





